Automata Learning for Automated Test Generation of Real Time Localization Systems

Cyber Physical Systems (CPSs) are often black box systems for which no exact model exists. Automata learning allows to build abstract models of CPSs and is used in several scenarios, i.e. simulation, monitoring, and test case generation. Real time localization systems (RTLSs) are an example of particularly complex and often safety critical CPSs. We present a procedure for automatic test case generation with automata learning and apply this approach in a case study to a localization system.

==> fig/black_box.tex <==
\begin{tikzpicture}[scale=0.8,transform shape]
    \node[draw, inner sep = 5pt, text width =1cm, align = center] at (0,0) (box) {$\tilde{q}$};
    \node at (-3,0) (in_ab) {$in$};
    \node at (3,0) (out_ab) {$out$};
    \node at (-1.5,0) (in) {$\tilde{in}$};
    \node at (1.5,0) (out) {$\tilde{out}$};
    %\node[above = 0.1cm of box] (func) {$\tilde{\beta}(i,q)$};

    \node[draw, text width = 3cm, inner sep = 15pt, dashed] at (0,0) (ab_box) {};

    \draw[->] (in) -- (box);
    \draw[->] (box) -- (out);
    \draw[->] (in_ab) -- (in);
    \draw[->] (out) -- (out_ab);
\end{tikzpicture}

==> fig/simple_example.tex <==
\begin{tikzpicture}[scale = 0.8,transform shape]
    \clip(-3,1) rectangle (3,-2.6);

    \node[circle, draw] at (0,0) (s2) {2};
    \node[circle, draw] at (0.5,-2) (s0) {0};
    \node[circle, draw] at (-1,-1.5) (s1) {1};

    \draw[->] (s0) -- (s1) node[midway,sloped,above] {S/b};
    \draw[->] (s1) -- (s2) node[midway,sloped,above] {E/b};
    \draw[->] (s2) -- (s0) node[midway,sloped,above] {S/a};

    \draw[->] (1.5,-1.2) -- (s0);

    \draw [->] (s0) to [out=50,in=-40] node[midway,sloped,above] {E/a} (s2);
    \draw [->] (s2) to [out=180,in=100] node[midway,sloped,above] {E/a} (s1);
    \draw [->] (s1) to [out=-60,in=200] node[midway,sloped,below] {S,N/a} (s0);
    \draw [->] (s0) to [out=0,in=-70,looseness=5] node[midway,right] {W,N/a} (s0);
    \draw [->] (s2) to [out=30,in=100,looseness=5] node[midway,above] {N/a} (s2);
\end{tikzpicture}
